Wireless-Powered Two-Way Relaying with Power Splitting-based Energy Accumulation

This paper investigates a wireless-powered two-way relay network (WP-TWRN), in which two sources exchange information with the aid of one amplify-and-forward (AF) relay. Contrary to the conventional two-way relay networks, we consider the scenario that the AF relay has no embedded energy supply, and it is equipped with an energy harvesting unit and rechargeable battery. As such, it can accumulate the energy harvested from both sources' signals before helping forwarding their information. In this paper, we develop a power splitting-based energy accumulation (PS-EA) scheme for the considered WP-TWRN. To determine whether the relay has accumulated sufficient energy, we set a predefined energy threshold for the relay. When the accumulated energy reaches the threshold, relay splits the received signal power into two parts, one for energy harvesting and the other for information forwarding. If the stored energy at the relay is below the threshold, all the received signal power will be accumulated at the relay's battery. By modeling the finite-capacity battery of relay as a finite-state Markov Chain (MC), we derive a closed-form expression for the system throughput of the proposed PS-EA scheme over Nakagami-m fading channels. Numerical results validate our theoretical analysis and show that the proposed PS-EA scheme outperforms the conventional time switching-based energy accumulation (TS-EA) scheme and the existing power splitting schemes without energy accumulation.

==> Distribution.tex <==
\section{Preliminary Statistics}
In this section, we present some important distributions for the harvested energy in Mode I or II and the outage-free relay transmit power of the relay for three adopted linear processing schemes in Mode III. Particularly, we derive closed-form expressions for the CDF of random variables $\tilde E_{\rm I}$ and $\tilde E_{\rm II}$ defined in (\ref{eq:harvested_enery_ModeI}) and (\ref{eq:harvested_enery_ModeII}), respectively. Moreover, the closed-form expressions for the CDF of random variables $P_R^{\rm X}$ defined in (\ref{eq:relay_power_threecase}) are also provided, where $\rm X \in \left\{{\rm MRC, ZF, MMSE}\right\}$ denotes the adopted linear processing schemes. These preliminary CDFs derived here will be used to characterize the performance of the considered system with ATF protocol in next section.

%The outage probability of the link $S-R$ is also characterized. In the following, we first characterize the distribution of the harvested energy in Mode I $\tilde E_{\rm I}$ given in (6).

\subsection{CDFs of $\tilde E_{\rm I}$ and $\tilde E_{\rm II}$}
As shown in (\ref{eq:harvested_enery_ModeI}), the harvested energy in Mode I, $\tilde E_{\rm I}$, can be regarded as a sum of the harvested energy from source, $E_{\rm{I,s}}= \frac{\eta}{2}{{P_0}{{\left\| {{{\bf{h}}_0}} \right\|}^2} }$, and the harvested energy from $L$ co-channel interferers, $E_{\rm{I,c}}= \eta \sum\nolimits_{l = 1}^L {{P_l}{{\left| {{h_l}} \right|}^2}}$. Since the entries in ${{{\bf{h}}_0}}$ suffers from i.i.d. Nakagami-m fading with the PDF given in (\ref{eq:PDF_nakagami_h0}), we can readily deduce that the harvested energy from source $E_{\rm{I,s}}$ is a gamma distributed random variable with shape parameter $m_sN_s$ and average power $\eta P_0 N_s \Omega_0 /2$. Similarly, the harvested energy from the interferers $E_{\rm{I,c}}$ is a weighted sum of $L$ gamma random variables with identical shape parameters $m_c$ and average powers $\eta P_l \Omega_l$, $l = 1,\ldots,L$. As such, we can treat $\tilde E_{\rm I}$ as a sum of $L+1$ mutually independent gamma random variables $\beta_j$, $j  = 1,\ldots,L +1$. That is, $\tilde E_{\rm I} = \sum\nolimits_{j = 1}^{L+1} {\beta_j}$ with
\begin{equation}
\beta_j = {\eta{P_j}{{\left| {{h_j}} \right|}^2}},~{\rm for}~j = 1, \cdots L ,~{\rm and}~{\beta_{L+1}} = E_{\rm{I,s}}. \end{equation}
We also have the corresponding shape parameters $ \left( {{m_1}, \cdots, {m_{L + 1}}} \right):$
\begin{equation}
{m_j} = {m_c},~{\rm for}~j = 1, \cdots L ,~{\rm and}~{m_{L+1}} = {m_s}{N_s} ,
\end{equation}
and average powers $\left( {{a _1}, \cdots, {a _{L + 1}}} \right):$
\begin{equation}
{a _j} = \eta P_{j} \Omega_{j},~{\rm for}~j = 1, \cdots L,~{\rm and}~{a_{L+1}} =\eta P_0 N_s \Omega_0 /2.
\end{equation}
However, to the best knowledge of the authors, it is very complicated to characterize a closed-form expression for the exact distribution of $\tilde E_{\rm I}$. Fortunately, by adopting a similar approach explored in \cite{Filho_EL_2004_Nak} and subsequently in \cite{Costa_CL_2011_Int,Costa_TVT_2012_Two}, we can tightly approximate the PDF of $\tilde E_{\rm I}$ (a sum of $L+1$ gamma random variables) by that of a single gamma random variable given by
\begin{equation}
\begin{split}
 {f_{\tilde E_{\rm I}}}\left( x \right)  \approx {{{m_I}^{{m_I}}{x^{{m_I} - 1}}} \over {\Gamma \left( {{m_I}} \right){\Omega _I}^{{m_I}}}}\exp \left( { - {{{m_I}} \over {{\Omega _I}}}x} \right),
  \end{split}
\end{equation}
where the parameters $m_I$ and $\Omega_I$ can be calculated by moment-based estimators. Specifically, we have
\begin{subequations}\label{}
\begin{align}
&{\Omega _I} = \mathbb{E}\left[ {{{\tilde E}_{\rm{I}}}} \right],\\
&{m_I} = \frac{{\Omega _I^2}}{{\mathbb{E}\left[ {{{\tilde E}_{\rm{I}}}^2} \right] - \Omega _I^2}}.
\end{align}
\end{subequations}
It is easily attain that ${\Omega _I} = \sum\limits_{j = 1}^{L+1} {a_j} $. To obtain the value of  $m_I$, a multinomial expansion is implemented to express the moment term $\mathbb{E}\left[ {{{\tilde E}_{\rm{I}}}^n} \right]$ in terms of the individual moments of the summands given by
%\begin{equation}
%{m_I} = {{{\Omega _I}^2} \over {\Phi  + {\Omega _I}^2}}.
%\end{equation}
%The parameter $\Phi$ in the above expression is given by
\begin{equation}
\begin{split}
\mathbb{E}\left[ {{{\tilde E}_{\rm{I}}}^n} \right]  & = \sum\limits_{{n_1} = 0}^n { \sum\limits_{{n_2} = 0}^{{n_1}} {\cdots  \sum\limits_{{n_L} = 0}^{{n_{L - 1}}} {\binom{n}{n_1}\binom{n_1}{n_2} \cdots \binom{n_{L-1}}{n_{L}}} } }\\
& \quad \times \mathbb{E}\left[ {\beta _1^{n - {n_1}}} \right]\mathbb{E}\left[ {\beta _2^{{n_1} - {n_2}}} \right] \cdots \mathbb{E}\left[ {\beta _{L + 1}^{{n_L}}} \right],
%\beta _1^{2\left( {n - {n_1}}\right)}\beta _2^{2\left( {n_1 - {n_2}}\right)}\cdots \beta _{L+1}^{2\left( { {n_{L-1}}} \right)},
\end{split}
\end{equation}
where
\begin{equation}
\mathbb{E}\left[\beta _j^n\right] = {{\Gamma \left( {{m_j} +  {n} } \right)} \over {\Gamma \left( {{m_j}} \right)}}{\left( {{{{a _j}} \over {{m_j}}}} \right)^{{n }}}.
\end{equation}
Based on the above result, the CDF of the harvested energy in Mode I can be approximated as
\begin{equation}\label{eq:CDF_EI}
\begin{split}
 {F_{\tilde E_{\rm I}}}\left( x \right)  \approx {{\gamma \left( {{m_I},{{{m_I}} \over {{\Omega _I}}}x} \right)} \over {\Gamma \left( {{m_I}} \right)}}.
  \end{split}
\end{equation}

We now turn to derive the statistics of the harvested energy in Mode II, i.e., $\tilde E_{\rm II}$. To this end, we first define the following random variable
\begin{equation}\label{}
  Y = \sum\limits_{l = 1}^L {{P_l}{{\left| {{h_l}} \right|}^2}}.
\end{equation}
We then have $\tilde E_{\rm II} = \frac{\eta}{2}Y$. Note that $Y$ is also included in the denominator of the received SINR at $R$ defined in (\ref{eq:SINR_R}).

Recall that in this paper we consider that all interfering links have distinct average power gains. The random variable $Y$ is thus a sum of $L$ independent gamma random variables with identical shape parameters $m_c$ and distinct average power $P_i \Omega_i$, $i = 1,\ldots,L$. With reference to \cite{Yu_TWC_2012_Out}, the PDF of the $Y$ can be found as
%We can also characterize the CDF of the harvested energy in Mode II ${F_{\tilde E_{\rm II}}}$ similarly from the above analysis. For the purpose of brevity, we omit this derivation in this paper.
\begin{equation}\label{eq:PDF_Y}
{f_Y}\left( y \right) = \sum\limits_{i = 1}^L {\sum\limits_{j = 1}^{{m_c}} {\frac{{{A_{i,j}}{y^{j - 1}}\exp \left( { - \frac{{{m_c}y}}{{{P_i}{\Omega _i}}}} \right)}}{{\left( {j - 1} \right)!}}} },
\end{equation}
where
\begin{equation}
\begin{split}
{A _{i,j}} &= {\left( { - 1} \right)^j}{\left( -{{{  {m_c}} \over {{P_i}{\Omega _i}}}} \right)^{{m_c}}}\sum\limits_{\tau \left( {i,j} \right)} {\prod\limits_{
   {k = 1},{k \ne i} }^L {\left( {\begin{matrix}
   {{m_c} + {q_k} - 1}  \\
   {{q_k}}  \\
 \end{matrix} } \right)}} \\
 &\quad \times {{{{\left( {{{{P_k}{\Omega _k}} \over {{m_c}}}} \right)}^{{q_k}}}} \over {{{\left( {1 - {{{P_k}{\Omega _k}} \over {{P_i}{\Omega _i}}}} \right)}^{{m_c} + {q_k}}}}},
 \end{split}
\end{equation}
and where ${\tau \left( {i,j} \right)}$ denotes a set of $p$-tuples such that ${\tau \left( {i,j} \right)} = \left\{ \left(q_1,\cdots,q_p\right) : q_k \in \mathbb{N}_0, \sum\nolimits_{k = 1}^p {{q_k} = {m_c} - j} \right\}$, with $\mathbb{N}_0$ representing the set of nonnegative integers. We now can obtain the CDF of $\tilde E_{\rm II}$ via
\begin{equation}\label{}
\begin{split}
 {F_{{{\tilde E}_{{\rm{II}}}}}}\left( x \right) &= \Pr \left( {{{\tilde E}_{{\rm{II}}}} < x} \right) = \Pr \left( {Y < \frac{{2x}}{\eta }} \right) \\
  &= \int_0^{\frac{{2x}}{\eta }} {{f_Y}\left( y \right)dy}  \\
 & = \sum\limits_{i = 1}^L {\sum\limits_{j = 1}^{{m_c}} {\frac{{{A_{i,j}}{{\left( {\frac{{{m_c}}}{{{P_i}{\Omega _i}}}} \right)}^j}\gamma \left( {j,\frac{{2x{m_c}}}{{\eta {P_i}{\Omega _i}}}} \right)}}{{\left( {j - 1} \right)!}}} },
  \end{split}
\end{equation}
where the integral is solved with the help of \cite[Eq. (3.351)]{Gradshteyn_book_2007}.

\subsection{CDF of ${P_R^{\rm X}}$}
In this subsection, we present the distribution of the required transmit power ${P_R^{\rm X}}$, $\rm X \in \left\{{\rm MRC, ZF, MMSE}\right\}$, for the three considered linear combining schemes at the destination. For notation simplicity, we define
\begin{equation}\label{eq:def_b}
b_l = P_l \Lambda_l, ~l \in \left\{1,\ldots,L\right\}.
\end{equation}
Recall that we consider distinct average channel power gains, i.e.,  ${{{b}}_i} \ne {b_j}$ when $ i\neq j $. Firstly, when MRC technique is implemented at the destination, the CDF of ${P_R^{\rm MRC}}$ can be calculated as
\begin{equation}\label{eq:CDF_MRC}
\begin{split}
{F_{\rm MRC}}\left( x \right) & = \Pr \left( {\frac{{\mu \left( {\sum\limits_{l = 1}^L {{P_l}\frac{{{{\left| {{\bf{g}}_0^\dag {{\bf{g}}_l}} \right|}^2}}}{{{{\left\| {{{\bf{g}}_0}} \right\|}^2}}}}  + \sigma _D^2} \right)}}{{{{\left\| {{{\bf{g}}_0}} \right\|}^2}}} < x} \right)\\
 &= \Pr \left( {\frac{{{{\left\| {{{\bf{g}}_0}} \right\|}^2}}}{{\sum\limits_{l = 1}^L {{P_l}\frac{{{{\left| {{\bf{g}}_0^\dag {{\bf{g}}_l}} \right|}^2}}}{{{{\left\| {{{\bf{g}}_0}} \right\|}^2}}}}  + \sigma _D^2}} > \frac{\mu }{x}} \right)\\
& = 1- {{\gamma \left( {{N_d},{{\mu {{\sigma _D}^2}} \over {x{\Lambda  _0}}}} \right)} \over {\Gamma \left( {{N_d}} \right)}} - \sum\limits_{i = 1}^L { {{{{\chi _{i}}{{\exp \left( {{{{{\sigma _D}^2}} \over {{b_i}}}} \right)}}} } } }\\
& \quad \times {{\Gamma \left( {{N_d},{{\mu {{\sigma _D}^2}} \over {{\Lambda _0}x}} + {{{{\sigma _D}^2}} \over {{b_i}}}} \right)} \over {{\Lambda _0}^{{N_d}}{{\left( {{1 \over {{\Lambda _0}}} + {x \over {\mu {b_i}}}} \right)}^{{N_d} }}\Gamma \left( {{N_d}} \right)}},
\end{split}
\end{equation}
where
\begin{equation}
{\chi _{i}} = {{{b_i}\prod\limits_{j = 1}^L {{1 \over {{b_j}}}} } \over {\prod\limits_{k = 1,k \ne i}^L {\left( {{1 \over {{b_k}}} - {1 \over {{b_i}}}} \right)} }}.
\end{equation}
where the last equality can be obtained by using the results given in \cite[Sec. II-C]{Romero_TWC_2008_Rece}.

%Note that when the interferering signals are statistically independent and identically distributed (i.i.d.), i.e. $b_i =b$, $\forall i \in 1,\cdots, L$. The CDF of ${P_R^{\rm MRC}}$ is given by
%\begin{equation}
%\begin{split}
%{F_{\rm MRC}}\left( x \right) &  = 1 - {{\gamma \left( {{N_d},{{\mu {\sigma ^2}} \over {x{\Lambda _0}}}} \right)} \over {\Gamma \left( {{N_d}} \right)}} - \sum\limits_{k = 0}^{L - 1} {\sum\limits_{l = 0}^k {{{\exp \left( {{{{\sigma ^2}} \over b}} \right){{\left( { - {\sigma ^2}} \right)}^{k - l}}} \over {l!\left( {k - l} \right)!{b^k}{{\left( {{\mu  \over x}} \right)}^l}}}} }\\
%& \quad \times {{\Gamma \left( {{N_d} + l,{{\mu {\sigma ^2}} \over {x{\Lambda _0}}} + {{{\sigma ^2}} \over b}} \right)} \over {{\Lambda _0}^{{N_d}}{{\left( {{1 \over {{\Lambda _0}}} + {x \over {\mu b}}} \right)}^{{N_d} + l}}\Gamma \left( {{N_d}} \right)}}.\\
%\end{split}
%\end{equation}
When the ZF technique is adopted at the destination, the co-channel interference will be completely eliminated. In this case, the destination will correspondingly lose the degree of freedom as the same as the number of interferers $L$. Hence, the CDF of ${P_R^{\rm ZF}}$ can be expressed as \cite{Zhu_TWC_2014_Out}
\begin{equation}\label{eq:CDF_ZF}
{F_{\rm ZF}}\left( x \right)  =  \sum\limits_{k = 0}^{N - L - 1} {{{{ \left( { {{\mu {\sigma _D}^2} \over \Lambda_0 x}} \right)^k}} \over {k!}}\exp \left( { - {{\mu {\sigma _D}^2} \over \Lambda_0 x}} \right)} .
\end{equation}

Finally, in terms of the MMSE scheme, we can have the CDF of ${P_R^{\rm MMSE}}$ given by
\begin{equation}\label{}
  {F_{\rm MMSE}} = \Pr\left\{ {\bf{g}}_0^\dag {\bf{R}}_I^{ - 1}{{\bf{g}}_0} > \frac{{\mu \sigma _D^2}}{x} \right\}.
\end{equation}
However, due to the complex structure of the term ${\bf{g}}_0^\dag {\bf{R}}_I^{ - 1}{{\bf{g}}_0}$, the closed-form expression for the CDF of ${P_R^{\rm MMSE}}$ can not be achieved  when the average channel gains (i.e., $b_l$'s defined in (\ref{eq:def_b})) of interferers are distinct. However, it is shown in \cite{Zhu_TWC_2014_Out} that the distribution can be well  approximated by the i.i.d. case, which corresponds to the scenario that the interferers are located in a cluster. By using the results provided in \cite{Zhu_TWC_2014_Out}, we can obtain an approximate closed-form expression for the CDF of ${P_R^{\rm MMSE}}$ given in (\ref{eq:CDF_MMSE}) on top of next page, in which ${}_2 {F_1}\left( {\alpha,\beta;\gamma;z} \right)$ is the Gauss hypergeometric function \cite[Eq. (9.10)]{Gradshteyn_book_2007} and $b = \left(\sum\nolimits_{l=1}^{L}{b_l}\right)/L$.
%the distribution of ${P_R^{\rm MMSE}}$ is given in (30) on the top of the next page.
%\newcounter{mytempeqncnt}
\begin{figure*}[!t]
% ensure that we have normalsize text
%\normalsize
\begin{equation}\label{eq:CDF_MMSE}
\begin{split}
{F_{\rm MMSE}}\left( x \right) \approx  {{\Gamma \left( {{N_d},{{\mu {\sigma _D}^2} \over {{\Lambda _0}x}}} \right)} \over {\Gamma \left( {{N_d}} \right)}} -& \Gamma \left( {L + 1} \right)\exp \left( { - {{\mu {\sigma _D}^2} \over {{\Lambda _0}x}}} \right){\left( {{{\mu {\sigma _D}^2} \over {{\Lambda _0}x}}} \right)^{{N_d}}}\times\\
&\sum\limits_{i = {\max \left( {0,N - L} \right) + 1}}^{{N_d}} {{{{{\left( {{b \over {{\sigma _D}^2}}} \right)}^{{N_d} - i + 1}}{}_2{F_1}\left( {L + 1,{N_d} - i + 1;{N_d} - i + 2; - {{\mu b} \over {{\Lambda _0}x}}} \right)} \over {\Gamma \left( i \right)\Gamma \left( {{N_d} - i + 2} \right)\Gamma \left( {i - {N_d} + L} \right)}}}.
\end{split}
\end{equation}
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}

%We now evaluate the outage probability of the first hop. With reference to [g4], the outage probability of the link $S-R$ can be expressed in (31) in the next page
%\newcounter{mytempeqncnt1}

%and the parameters
%
%\setcounter{mytempeqncnt}{\value{equation}}
%\setcounter{equation}{31}
%When the interferering signals are statistically i.i.d., i.e. $P_i \Omega_i =a$, $\forall i \in 1,\cdots, L$.
% The outage probability of the first hop is given by
%\begin{equation}
%\begin{split}
%\varphi & = 1 - \exp \left( { - {{{m_s}{\sigma ^2}\mu } \over {{P_0}{\Omega _0}}}} \right) {\left( {{{{m_r}} \over a}} \right)^{{m_r}L}}\sum\limits_{k = 0}^{{m_s}{N_s} - 1} {{{{{\left( {{{{m_s}\mu } \over {{\Omega _0}}}} \right)}^k}} \over {\Gamma \left( {{m_r}L} \right)k!}}} \\
%& \quad \times \sum\limits_{l = 0}^k {{{{{\binom{k}{l}\left( {{\sigma ^2}} \right)}^{k - l}}\left( {m_r L - 1 + l} \right)!} \over {{{\left( {{{{m_r}} \over {a}} + {{{m_s}\mu } \over {{P_0}{\Omega _0}}}} \right)}^{m_r L + l}}}}} .
%\end{split}
%\end{equation}




